Robust Inference for High-dimensional Linear Models with Heavy-tailed Errors via Partial Gini Covariance

This paper introduces the partial Gini covariance, a novel dependence measure that addresses the challenges of high-dimensional inference with heavy-tailed errors, often encountered in fields like finance, insurance, climate, and biology. Conventional high-dimensional regression inference methods suffer from inaccurate type I errors and reduced power in heavy-tailed contexts, limiting their effectiveness. Our proposed approach leverages the partial Gini covariance to construct a robust statistical inference framework that requires minimal tuning and does not impose restrictive moment conditions on error distributions. Unlike traditional methods, it circumvents the need for estimating the density of random errors and enhances the computational feasibility and robustness. Extensive simulations demonstrate the proposed method's superior power and robustness over standard high-dimensional inference approaches, such as those based on the debiased Lasso. The asymptotic relative efficiency analysis provides additional theoretical insight on the improved efficiency of the new approach in the heavy-tailed setting. Additionally, the partial Gini covariance extends to the multivariate setting, enabling chi-square testing for a group of coefficients. We illustrate the method's practical application with a real-world data example.

==> definition.tex <==
\usepackage{latexsym, amsbsy, amssymb,multirow, epsfig, amsmath}
\usepackage{comment}
\usepackage{hyperref}

%--------------------Initialize---------------------%
%\textheight= 9in  \textwidth = 6.5in \topmargin = -1.4cm
%\oddsidemargin = -0.15in \evensidemargin = 0in
%\usepackage{natbib,graphicx,setspace,lscape,longtable}
\usepackage{natbib,epsfig,graphicx}
\usepackage{subfigure}
%\usepackage{floatrow}   
\usepackage{tikz}
%\usepackage{subcaption}
\usepackage{xcolor} 
\usepackage[framemethod=tikz]{mdframed}
\usepackage{amsmath,amsthm,amssymb,color}
\usepackage{makecell}
\RequirePackage[mathlines, displaymath]{lineno}
\bibpunct{(}{)}{;}{a}{,}{,}

%\setlength{\textwidth}{6.2in} \setlength{\textheight}{8.75in}
%\setlength{\topmargin}{-0.25in} \setlength{\oddsidemargin}{0.25in}
%\setlength{\evensidemargin}{0.25in}
%%%%%%%%

%------------ Yilin Zhang's Definition ---------------%


%%%%%%%%%%%%%%%%%%%%%
%\newtheorem{theorem}{Theorem}
%\newtheorem{lemma}{Lemma}
%\newtheorem{prop}{Proposition}
%\baselineskip = 7mm
%\parskip = 2.5mm




\def\beqr{\begin{eqnarray}}
\def\eeqr{\end{eqnarray}}
\def\beqrs{\begin{eqnarray*}}
\def\eeqrs{\end{eqnarray*}}
\def\bep{\begin{prop}}
\def\eep{\end{prop}}

\def\mR{\mathbb{R}}
\def\calA{\mathcal{A}}
\def\calB{\mathcal{B}}
\def\calC{\mathcal{C}}
\def\calD{\mathcal{D}}
\def\calF{\mathcal{F}}
\def\calI{\mathcal{I}}
\def\calS{\mathcal{S}}
\def\calG{\mathcal{G}}
\def\calP{\mathcal{P}}
\def\calM{\mathcal{M}}
\def\calL{\mathcal{L}}
\def\calN{\mathcal{N}}
\def\calU{\mathcal{U}}
\def\calT{\mathcal{T}}
\def\calH{\mathcal{H}}
\def\calR{\mathcal{R}}
\def\calX{\mathcal{X}}
\def\calY{\mathcal{Y}}
\def\calZ{\mathcal{Z}}
\def\calV{\mathcal{V}}

%\newtheorem{Theorem}{Theorem}[section]
%\newtheorem{Corollary}{Theorem}[section]
%\newtheorem{Lemma}[Theorem]{Lemma}




\def\bias{\mbox{bias}}
\def\pr{\mbox{pr}}
\def\var{\mbox{var}}
\def\cov{\mbox{cov}}
\def\cor{\mbox{cor}}
\def\MSE{\mbox{MSE}}
\def\arcos{\mbox{arcos}}

%\textheight= 9in
%\textwidth = 6.1in
%\evensidemargin = 0in
%\renewcommand{\thefootnote}{\fnsymbol{footnote}}


%\numberwithin{equation}{section}
%\renewcommand{\baselinestretch}{1.75}


%\bibliographystyle{cheng}
%\renewcommand\refname{REFERENCE}
%\bibliographystyle{refstyle}
%\renewcommand\refname{REFERENCE}


%-------------Li-Ping's Definition-----------------------%

\def\wh{\widehat}
\def\wt{\widetilde}
\def\ba{\mbox{\boldmath$\alpha$}}
\def\bphi{\mbox{\boldmath$\phi$}}
\def\bb{\mbox{\boldmath$\beta$}}
\def\bg{\mbox{\boldmath$\gamma$}}
\def\ha{\mbox{$\widehat\ba$}}
\def\hb{\mbox{$\widehat\bb$}}
\def\hg{\mbox{$\widehat\bg$}}
\def\gg{>\!\!>}
\def\ll{<\!\!<}
\def\hDash{\bot\!\!\!\bot}
\def\nhDash{\not\!\perp\!\!\!\perp}


\def\a{{\bf a}}
\def\b{{\bf b}}
\def\A{{\bf A}}
\def\B{{\bf B}}
\def\C{{\bf C}}
\def\V{{\bf V}}
\def\G{{\bf G}}
\def\X{{\bf X}}
\def\x{{\bf x}}
\def\Y{{\bf Y}}
\def\y{{\bf y}}
\def\Z{{\bf Z}}
\def\z{{\bf z}}
\def\u{{\bf u}}
\def\s{{\bf s}}
\def\t{{\bf t}}
\def\h{{\bf h}}
\def\k{{\bf k}}
\def\l{{\bf l}}
\def\c{{\bf c}}
\def\v{{\bf v}}
\def\d{{\bf d}}
\def\w{{\bf w}}
\def\g{{\bf g}}
\def\I{{\bf I}}
\def\R{{\bf R}}
\def\P{{\bf P}}
\def\vo{{\bf 1}}
\def\vz{{\bf 0}} 

\def\balpha{{\bm \alpha}}
\def\bbeta{{\bm \beta}}
\def\btheta{{\bm \theta}}
\def\bgamma{{\bm \gamma}}
\def\bzeta{{\bm \zeta}}
\def\betaa{{\bm \eta}}
\def\bome{{\bm \omega}}
\def\bpi{{\bm \pi}}

\newcommand{\trans}{^\top}%{^{\mbox{\tiny{T}}}}
\def\defby{\stackrel{\mbox{\textrm{\tiny def}}}{=}}

\newcommand{\beps}{\mbox{\boldmath $\varepsilon$}}
\newcommand{\bSig}{\mbox{\boldmath $\Sigma$}}
\newcommand{\hSig}{\mbox{$\widehat{\bSig}$}}
\newcommand{\bLam}{\mbox{\boldmath $\Lambda$}}
\newcommand{\hLam}{\mbox{$\widehat{\bLam}$}}
\newcommand{\bOmega}{\mbox{\boldmath $\Omega$}}
\newcommand{\bI}{\mbox{\boldmath $I$}}
\newcommand{\bGam}{\mbox{\boldmath $\Gamma$}}

\newtheorem{defi}{\sc Definition}[section]
\newtheorem{theo}{\bf Theorem}
\newtheorem{lemm}{\sc Lemma}
\newtheorem{prop}{\sc Proposition}
\newtheorem{coll}{\sc Corollary}[theo]
\newtheorem{rema}{\bf Remark}
\newtheorem{exam}{\bf Example}



\def\diamondplus{\mathrel{%
		\ooalign{\raise.29ex\hbox{$\scriptscriptstyle+$}\cr\hss$\diamond$\hss}}}

%--------------------------------------------------------------%

% double tilde

\usepackage{calc}

\usepackage{accents}
\newcommand{\dbtilde}[1]{\accentset{\approx}{#1}}
\newcommand{\vardbtilde}[1]{\tilde{\raisebox{0pt}[0.85\height]{$\tilde{#1}$}}}



\newcommand{\FDR}{\mathrm{FDR}}
\newcommand{\FDP}{\mathrm{FDP}}

\newcommand{\skipline}{\vspace{12pt}}
\newcommand{\Rcor}{{\rm{Rcor}}}
\newcommand{\Scor}{{\rm{Scor}}}
\newcommand{\Dcov}{{\rm{Dcov}}}
\newcommand{\Qcov}{{\rm{Qcov}}}
\newcommand{\Gcov}{{\rm{Gcov}}}
\newcommand{\pGcov}{{\rm{pGcov}}}
\newcommand{\pQcov}{{\rm{pQcov}}}
\newcommand{\pCQcov}{{\rm{pCQcov}}}
\newcommand{\pPcov}{{\rm{pPcov}}}
\newcommand{\Acov}{{\rm{Acov}}}
\newcommand{\DC}{{{\rm DC}}}
\newcommand{\PC}{{{\rm PC}}}
\newcommand{\AC}{{{\rm AC}}}
\newcommand{\BPC}{{{\rm BPCor}}}
\newcommand{\PCPR}{{{\rm PCPR}}}
\newcommand{\HSIC}{{{\rm HSIC}}}
\newcommand{\ARE}{{\rm{ARE}}}

\newcommand{\dBeta}{{\rm{dBeta}}}

\newcommand{\D}{\mbox{D}}
\newcommand{\E}{\mbox{E}}
\newcommand{\diff}{\mbox{d}}
\newcommand{\F}{\mbox{F}}
\newcommand{\NLS}{\mbox{NLS}}
\newcommand{\GPLSIM}{\mbox{GPLSIM}}
\newcommand{\Known}{\mbox{Known}}
\newcommand{\PS}{\mbox{PS}}
\newcommand{\PR}{\mbox{PR}}
\newcommand{\LS}{\mbox{LS}}
\newcommand{\LSR}{\mbox{LSR}}
\newcommand{\PPR}{\mbox{PPR}}
\newcommand{\SIR}{\mbox{SIR}}
\newcommand{\pHd}{\mbox{pHd}}
\newcommand{\tr}{\mbox{tr}}
\newcommand{\vech}{\mbox{vech}}
\newcommand{\mvz}{\mbox{${\bf z}$}}
\newcommand{\Hessian}{\mbox{${\bf H}$}}

\newcommand{\ang}{{\rm{ang}}}


\newcommand{\yvec}{\mbox{\boldmath $y$}}

\newcommand{\Zvec}{\mbox{\boldmath $Z$}}
\newcommand{\avec}{\mbox{\boldmath $a$}}
\newcommand{\bvec}{\mbox{\boldmath $b$}}
\newcommand{\mvec}{\mbox{\boldmath $m$}}
\newcommand{\svec}{\mbox{\boldmath $s$}}
\newcommand{\tvec}{\mbox{\boldmath $t$}}
\newcommand{\uvec}{\mbox{\boldmath $u$}}
\newcommand{\wvec}{\mbox{\boldmath $w$}}
\newcommand{\gammavec}{\mbox{\boldmath $\gamma$}}
\newcommand{\epsvec}{\mbox{\boldmath $\epsilon$}}
\newcommand{\zetavec}{\mbox{\boldmath $\zeta$}}
\newcommand{\etavec}{\mbox{\boldmath $\eta$}}
\newcommand{\thetavec}{\mbox{\boldmath $\theta$}}
\newcommand{\chivec}{\mbox{\boldmath $\chi$}}
\newcommand{\Covmat}{\mbox{\boldmath $\Sigma$}}
\newcommand{\Bmat}{\mbox{${\bf B}$}}
% \newcommand{\norm}{\|} % commented by ccy
\usepackage{latexsym}
\usepackage{epsfig}
\usepackage{bm}

\usepackage{threeparttable}
\usepackage{booktabs}
%\usepackage{siunitx,booktabs} % table row space
%\sisetup{separate-uncertainty}
%\renewcommand{\baselinestretch}{1.75}
%
%\newcommand{\csection}[1]
%{\begin{center}
%		\stepcounter{section}
%		{\bf\large\arabic{section}. #1}
%	\end{center}
%	\vspace{-0.15 cm}}
%\newcommand{\scsection}[1]
%{\begin{center}
%		{\bf\large #1}
%	\end{center}
%	\vspace{-0.15 cm}}
%\newcommand{\csubsection}[1]{
%	\vspace{-0.25 cm}
%	\begin{center}
%		\stepcounter{subsection}
%		{\it\arabic{section}.\arabic{subsection}. #1}
%	\end{center}
%	\vspace{-0.25 cm}}
%\newcommand{\scsubsection}[1]{
%	\vspace{-0.25 cm}
%	\begin{center}
%		\stepcounter{subsection}
%		{\it #1}
%	\end{center}
%	\vspace{-0.25 cm}}
%
%
%
%
%%\usepackage{xr}
%%\externaldocument{其他文件名称，可以引用其他文件中出现的标号} % 例如，
%\usepackage{xr}
%\externaldocument{chap1}
%% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
%%                      																								  %
%%                      					可能需要使用特殊的一些包    			    			 %
%%                      																								  %
%% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
%\RequirePackage[mathlines, displaymath]{lineno}
%\usepackage{natbib}
%\usepackage{latexsym, amsbsy, amssymb,multirow, epsfig, amsmath}
%\usepackage[left=30mm,right=28mm,top=2cm,bottom=2cm]{geometry}
%%\usepackage{amssymb,amsthm,amsmath,mathrsfs,bm,color}
%%\setlength{\textwidth}{6.2in} \setlength{\textheight}{8.75in}
%%\setlength{\topmargin}{-0.25in} \setlength{\oddsidemargin}{0.25in}
%%\setlength{\evensidemargin}{0.25in}
%%\usepackage{hyperref}
%%\baselineskip = 7mm
%%\parskip = 2.5mm
%%
%%\textheight= 9in
%%\textwidth = 6.1in
%%\evensidemargin = 0in
%%
%
%
%% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
%%                      																								  %
%%                      					可能需要使用特殊的命令行    			    			 %
%%                      																								  %
%% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
%\def\beqr{\begin{eqnarray}}
%\def\eeqr{\end{eqnarray}}
%\def\beqrs{\begin{eqnarray*}}
%\def\eeqrs{\end{eqnarray*}}
%
%% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
%%                      																								  %
%%                      					给出比较常用的定理环境定义  	   	   	    			 %
%%                      																								  %
%% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
%\newtheorem{theo}{\bf Theorem}
%\bibliographystyle{refstyle}
%\renewcommand\refname{REFERENCE}
%
%% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
%%                      																								  %
%%                      					给出比较常用的特殊算子定义  		   	    			 %
%%                      																								  %
%% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
%\def\pr{\mbox{pr}}
%\def\cov{\mbox{cov}}
%\def\var{\mbox{var}}
%\def\sign{\mbox{sign}}
%\def\sp{\textrm{span}}
%\def\vecl{\textrm{vecl}}
%
%
%
%% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
%%                      																								  %
%%                      					给出比较常用的特殊符号定义  		   	    			 %
%%                      																								  %
%% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
%\def\mR{\mathbb{R}}
%\def\calA{\mathcal{A}}
%\def\calB{\mathcal{B}}
%\def\calC{\mathcal{C}}
%\def\calD{\mathcal{D}}
%\def\calI{\mathcal{I}}
%\def\calN{\mathcal{N}}
%\def\calS{\mathcal{S}}
%\def\calX{\mathcal{X}}
%\def\calY{\mathcal{Y}}
%\def\calZ{\mathcal{Z}}
%
%
%\def\a{{\bf a}}
%\def\b{{\bf b}}
%\def\c{{\bf c}}
%\def\d{{\bf d}}
%\def\u{{\bf u}}
%\def\v{{\bf v}}
%\def\w{{\bf w}}
%\def\x{{\bf x}}
%\def\y{{\bf y}}
%\def\z{{\bf z}}
%
%\def\A{{\bf A}}
%\def\B{{\bf B}}
%\def\C{{\bf C}}
%\def\D{{\bf D}}
%\def\I{{\bf I}}
%\def\X{{\bf X}}
%\def\Y{{\bf Y}}
%\def\Z{{\bf Z}}
%
%
%\def\ba{\mbox{\boldmath$\alpha$}}
%\def\bb{\mbox{\boldmath$\beta$}}
%\def\bSig{\mbox{\boldmath$\Sigma$}}
%
%% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
%%                      																								  %
%%                      					给出其他一些的特殊算子定义  		   	    			 %
%%                      																								  %
%% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
%\def\defby{\stackrel{\mbox{\textrm{\tiny def}}}{=}}
%\newcommand{\trans}{^{\mbox{\tiny{T}}}}
%\def\hDash{\bot\!\!\!\bot}
%\def\wh{\widehat}
%\def\wt{\widetilde}



% --------------- Added by ccy ----------------------- %
% norm & abs
\newcommand{\norm}[1]{\Vert#1\Vert}
\newcommand{\Norm}[1]{\left\Vert#1\right\Vert}
\newcommand{\inner}[2]{\langle #1, #2 \rangle}
\newcommand{\Inner}[2]{\left\langle #1, #2 \right\rangle}
\newcommand{\abs}[1]{\vert#1\vert}
\newcommand{\Abs}[1]{\left\vert#1\right\vert}


\usepackage{enumitem} % redefine enumerate


\usepackage[colorinlistoftodos]{todonotes} % for todo

\usepackage{tikz}

\usepackage{amssymb}


\usepackage{threeparttable}
\usepackage{multirow}

% for caption below table, cf. https://latex.org/forum/viewtopic.php?t=5572.
\usepackage{caption}


\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}

\DeclareMathOperator\supp{supp}



==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}
